Spores: Stateless Predictive Onion Routing for E-Squads

Mass surveillance of the population by state agencies and corporate parties is now a well-known fact. Journalists and whistle-blowers still lack means to circumvent global spying for the sake of their investigations. With Spores, we propose a way for journalists and their sources to plan a posteriori file exchanges when they physically meet. We leverage on the multiplication of personal devices per capita to provide a lightweight, robust and fully anonymous decentralised file transfer protocol between users. Spores hinges on our novel concept of e-squads: one's personal devices, rendered intelligent by gossip communication protocols, can provide private and dependable services to their user. People's e-squads are federated into a novel onion routing network, able to withstand the inherent unreliability of personal appliances while providing reliable routing. Spores' performances are competitive, and its privacy properties of the communication outperform state of the art onion routing strategies.

==> Makefile <==
.PHONY: all viewpdf pdf clean

TARGET       = main
SOURCE_FILES = $(shell find . -type f -name "*.tex" -print)
#SOURCE_FILES = $(TARGET).tex $(wildcard */*.tex)
BIB_FILES    = $(shell find . -type f -name "*.bib" -print)
FIGURES      = $(shell find . -path "*/figures/*" -type f -print)

#BIB_PROCESSOR := biber
BIB_PROCESSOR := bibtex

# Set the pdf reader according to the operating system
OS = $(shell uname)
ifeq ($(OS), Darwin)
	PDF_READER = open
endif
ifeq ($(OS), Linux)
	PDF_READER = evince
endif

all: pdf
	
viewpdf: pdf
	$(PDF_READER) $(TARGET).pdf &

pdf: $(TARGET).pdf

$(TARGET).pdf: $(SOURCE_FILES) $(BIB_FILES) $(FIGURES)
	pdflatex -interaction=nonstopmode -jobname=$(TARGET) $(TARGET).tex
	$(BIB_PROCESSOR) $(TARGET)
	pdflatex -interaction=nonstopmode -jobname=$(TARGET) $(TARGET).tex # For biber
	pdflatex -interaction=nonstopmode -jobname=$(TARGET) $(TARGET).tex # For biber

clean:
	@for suffix in dvi aux bbl blg toc ind out brf ilg idx synctex.gz log run.xml bcf ps; do \
		find . -name "*.$${suffix}" -delete; \
	done
	#@rm $(TARGET).pdf

